Community detection using fast low-cardinality semidefinite programming

Modularity maximization has been a fundamental tool for understanding the community structure of a network, but the underlying optimization problem is nonconvex and NP-hard to solve. State-of-the-art algorithms like the Louvain or Leiden methods focus on different heuristics to help escape local optima, but they still depend on a greedy step that moves node assignment locally and is prone to getting trapped. In this paper, we propose a new class of low-cardinality algorithm that generalizes the local update to maximize a semidefinite relaxation derived from max-k-cut. This proposed algorithm is scalable, empirically achieves the global semidefinite optimality for small cases, and outperforms the state-of-the-art algorithms in real-world datasets with little additional time cost. From the algorithmic perspective, it also opens a new avenue for scaling-up semidefinite programming when the solutions are sparse instead of low-rank.

==> Makefile <==
MAIN := lowcard
all: $(MAIN).pdf
	#open $(MAIN).pdf

$(MAIN).pdf: $(MAIN).tex sdp.bib
	pdflatex $(MAIN)
	bibtex $(MAIN)
	pdflatex $(MAIN)
	pdflatex $(MAIN)
	#@latexmk -pdf -dvi- -ps- -use-make -quiet #\
	#-pdflatex='pdflatex -interaction=batchmode --shell-escape  %O %S' $<

.PHONY: install
install:
	open $(MAIN).pdf &

.PHONY: clean
clean:
	latexmk -bibtex -C

